Data Synthesis for Testing Black-Box Machine Learning Models

The increasing usage of machine learning models raises the question of the reliability of these models. The current practice of testing with limited data is often insufficient. In this paper, we provide a framework for automated test data synthesis to test black-box ML/DL models. We address an important challenge of generating realistic user-controllable data with model agnostic coverage criteria to test a varied set of properties, essentially to increase trust in machine learning models. We experimentally demonstrate the effectiveness of our technique.

==> arch.tex <==
\section{Architecture}
\label{sec:arch}


\begin{figure}[t]
\centering
\includegraphics[height=3.5cm, width=8cm]{images/aitestingarch.png}
\caption{\system{} Architecture}
\label{fig:arch}
\vspace{-7mm}
\end{figure}

Figure~\ref{fig:arch} shows the different components of \system{} architecture and how they interact with each other. Next, we summarize the functionalities of different components of \system{} with a toy example.  

{\bf Training Data}.  Consider a toy dataset (row count 1000) with  \begin{wraptable}{r}{2.5cm}
\scriptsize
\begin{tabular}{ccc}
gender & salary & loan\\\hline
M & 0 &  0\\
F & 12 &  0\\
...&... &...
\end{tabular}
\end{wraptable}
two attributes (\texttt{gender}, \texttt{salary}) and 
the binary label \texttt{loan} where 0 signifying loan is not granted, and 1 otherwise.  
% The number of rows is 1000.


\noindent{\bf Constraint Inference.}  The constraint inference engine analyzes the training data with additional input of the label attribute.  It infers the following feature and association constraints:\\


\begin{minipage}[b]{0.2\textwidth}
\hspace{-20pt}
\includegraphics[width=3cm]{images/gender-histogram-plt.png}
\end{minipage}
%\hfill
\hspace{-20pt}
\begin{minipage}[b]{0.2\textwidth}
\hspace{-20pt}
\includegraphics[width=3cm]{images/salary-plt.png}
%\includegraphics[width=3cm]{images/gender-salary.png}
\end{minipage}
%\hfill
\hspace{-20pt}
\begin{minipage}[b]{0.2\textwidth}
\hspace{-20pt}
\includegraphics[width=3cm]{images/gender-salary-plt.png}
%\includegraphics[width=3cm]{images/gender-salary.png}
\end{minipage}\\

% \begin{minipage}[b]{0.2\textwidth}
% \includegraphics[width=4cm]{images/gender-histogram.png}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.2\textwidth}
% \includegraphics[width=4cm]{images/gender-salary.png}
% \end{minipage}\\

% \begin{minipage}[b]{0.2\textwidth}
% \includegraphics[width=4cm]{images/male-salary.png}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.2\textwidth}
% \includegraphics[width=4cm]{images/female-salary.png}
% \end{minipage}\\

% \begin{minipage}[b]{0.2\textwidth}
% \includegraphics[width=4cm]{images/loan-salary.png}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.2\textwidth}
% \includegraphics[width=4cm]{images/loan-gender.png}
% \end{minipage}\\
 
\noindent{\bf User-specified Constraints.} Say, user specifies the ratio of M and F to be 1:1, overriding the frequency distribution in the data.

\noindent{\bf Decision Tree Surrogate Builder and coverage constraint extractor.}  This step builds a decision tree model approximating the target model. Constraint extractor ANDs all constraints in a path to create the path-constraints corresponding to each path in the decision tree.  A sample decision-tree along with its four path constraints which are used in the coverage based data synthesis are shown below.

\begin{minipage}[b]{0.2\textwidth}
\includegraphics[width=4cm]{DT.JPG}
\end{minipage}
\hfill
\begin{minipage}[b]{0.2\textwidth}
\scriptsize
$Gender = F$ \& $Salary < 6$\\
$Gender = F$ \& $Salary \ge 6$\\
$Gender = M$ \& $Salary < 10$\\
$Gender = M$ \& $Salary >= 10$\\
\end{minipage}\\

\noindent{\bf Constraint Merger.}  Constraint merger is responsible for merging user-specified constraints into data constraints. In this case, it will overwrite the Male-Female ratio.

\noindent{\bf Accuracy Test-case Generator.}  To generate accuracy-test cases, \system{} uses a custom constraint solver to satisfy the constraints obtained from data/user-specified/coverage constraints  \begin{wraptable}{r}{2cm}
\scriptsize
\begin{tabular}{cc}
gender & salary\\\hline
M & 1\\
F & 13\\
\end{tabular}
\end{wraptable}
and generates the specified number of samples. Testing accuracy also requires ground-truth labels for the generated samples. Generating labels requires human involvement and is used whenever they are available. Otherwise, we use a labeler, as presented below.  Satisfying the above constraints, the generated samples are shown in the right. 

\noindent{\bf Labeler.} \system{} uses a novel approach to approximate human labels for the generated samples. The approach, in Section~\ref{subsec:accuracy}}, assigns labels to corresponding samples based on high-confidence voting of many models built from the training data. 

\noindent{\bf Adversarial Robustness Test-case Generator.}  This will generate pairs of samples  as shown in right (by slightly perturbing 
\begin{wraptable}{r}{2cm}
\scriptsize
\begin{tabular}{cc}
gender & salary\\\hline
M & 9\\
M & 10\\
\end{tabular}
\end{wraptable} 
  attribute values). Note that, if the coverage model is accurate, then this
 pair of samples will return different labels signifying violation of robustness. 


\noindent{\bf Group Fairness Test-case Generator.}
Fairness test case generator requires additional input for fairness specification, which involves the specification of protected attributes. In this case, say \texttt{gender}, a protected attribute with privileged group 'Male' is defined by the expression $gender = M$ and un-privileged group 'Female' as $gender = F$ with favorable outcome $loan = 1$ signifying loan granted.  Based on solving data constraints and user-specific constraints, the required number of samples is generated. Generally, more realistic samples will give a better idea of discrimination present in the model.

\noindent{\bf Individual Fairness Test-case Generator.} This will create pairs \begin{wraptable}{r}{2cm}
\scriptsize
\begin{tabular}{cc}
gender & salary\\\hline
M & 6\\
F & 6\\
\end{tabular}
\end{wraptable} 
of samples satisfying all three types of constraints. Note that, if the coverage model is accurate, then this pair of samples will return different labels signifying discrimination. 



==> constraints_inference_algo.tex <==
% !TEX root = main.tex
\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon


 \SetKwFunction{FMain}{get\_constraints}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{data}}{ \label{func:get_constraints}
   datatypes = get\_datatypes(data) \\
   col\_constraints = get\_column\_constraints(data, datatypes) \\
   associations = get\_associations(data, datatypes) \\
%        \KwRet
  }

  \SetKwFunction{FMain}{get\_datatypes}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{column\_data}}{ \label{func:get_datatypes}
%      \ForEach {column $c$ in data}{ \label{line:r11x}
        num\_values = size(column\_data)\\
        num\_uniques\_values = size(unique(column\_data)))  \\
        \lIf {num\_values = 0} {\Return{EMPTY}}
	\lIf {has\_real\_values(column\_data)} {\Return{FLOAT}}
         \lIf {has\_date\_values(column\_data)} {\Return{DATE}}
	   \eIf {num\_unique\_values < max(log (num\_values), 20)}{
		\uIf {has\_int\_values(column\_data)} {
			\Return{CAT\_NUM}\\
		}
		\Return{CAT\_TEXT}
		
	}{
		\uIf {has\_int\_values(column\_data)} {
			\Return{NUMERIC}
		}
		\Return{TEXT}
	}
%     }
%        \KwRet\;
  }


   \SetKwFunction{FMain}{get\_column\_constraints}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{data}}{ 
  \label{func:get_column_constraints}
      \ForEach {column $c$ in data}{
	$dt$ = get\_datatype(c.data)\\
%     	 \If{dt \in (\set{CAT\_NUM, CAT\_CAT})} {
	 \uIf{$dt$ $\in$ (CAT\_NUM, CAT\_TEXT)} {
      		c.frequency = frequency\_distribution(c.values)
      	}
      	\uElseIf{$dt$ $\in$ (NUMERIC, FLOAT)} {
      		c.min = min(c.values)\\
		c.max = max(c.values)\\
		c.mean = mean(c.values)\\
		c.dist = distribution(c.values)
        }\uElseIf{$dt$ = DATE}{
        		c.start\_date = mindate(c.values)\\
		c.end\_date = maxdate(c.values)\\
		c.format = get\_format(c.values)
        }
%
     }
%        \KwRet\;
  }
  \caption{Constraints Inference}\label{algo:constraints}
  
\end{algorithm}



\begin{algorithm}
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon
%  \setcounter{AlgoLine}{38}
  \SetKwFunction{FMain}{get\_associations}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{data}}{ 
  \label{func:get_associations}
  	association\_list = empty \\
      \ForEach {columns $c_1,c_2$ in data}{
%       \ForEach {column $c_2$ in data}{
	association a\\
	a.source = $c_1$\\
    	a.target = $c_2$\\
      	$dt_1$ = get\_datatype($c_1$)\\
	$dt_2$ = get\_datatype($c_2$)\\
	\uIf{$dt_1 \in$ (CAT\_NUM, CAT\_CAT)} {
	 \uIf{$dt_2 \in$ (CAT\_NUM, CAT\_CAT)} {
		a.type = CAT-CAT\\
%		association.subtype = FREQUENCY-DIST\\
%		catcat\_list = empty\\
		 \ForEach {v in $c_1$}{
%		 	a.type = CAT-CAT\\
		 	target\_vals = get\_target\_vals(v)\\
			a.src\_value = v\\
			a.frequency = get\_freq(target\_vals)  \\
			association\_list.add(a)
%		 	catcat.src\_value = v\\
%			catcat.freq = get\_freq(target\_vals) \\
%		 	catcat\_list.add(catcat)
		 }
%		 association.frequency = catcat\_list\\
%		 association\_list.add(association)
		 }
     
         \uElseIf{$dt_2 \in$ (NUMERIC, FLOAT)}{
     	a.type = CAT-NUM\\
%		association.subtype = RANGEPOLYNOMIAL\\
%		catnum\_list = empty\\
		 \ForEach {v in $c_1$}{
		 	target\_vals = get\_target\_vals(v, $c_2$) \\
			a.src\_value = v \\
			a.dist, a.error = get\_dist(target\_values)\\
			association\_list.add(a)
%			catnum.src\_value = v \\
%			catnum.dist = get\_dist(target\_values)\\
%			catnum\_list.add(catnum)
		 }
%		 association.polynomials = catnum\_list\\
%		 association\_list.add(association)
         }}
         \uElseIf{$dt_1 \in$ (NUMERIC, FLOAT)} {
	 \uIf{$dt_2 \in$ (NUMERIC, FLOAT)} {
	 	a.type = NUM-NUM\\
%		a.subtype = POLYNOMIAL\\
		 a.poly, a.error = get\_polynomial($c_1,c_2$)\\
		 association\_list.add(a)\\
		 \ForEach{category column $c_3$ in data}{
		 
%		 	$d_3$ = get\_datatype($c_3$)\\
%		 	\If{$d_3 \in$ (CAT\_NUM,CAT\_TEXT) }{
				a.type = CAT-NUM-NUM\\
				a.catcol = $c_3$ \\
%				cnn\_list = empty\\
				\ForEach {v in $c_3$.data}{
					$v_1$= get\_target\_vals(v, $c_1$) \\
					$v_2$= get\_target\_vals(v, $c_2$) \\
%					cnn.src\_val = $v$\\
					a.poly, a.error = get\_polynomial($v_1,v_2$)\\
					association\_list.add(a)
%					cnn\_list.add(cnn)
%				}
			}
%			association.polynomials = cnn\_list\\
%			 association\_list.add(association)

		 }
	 }}
%         \If{$dt_1 \in$ (DATE) $\wedge$ $dt_2 \in$ (DATE)}{
%         
%         }
         
%
     }
%     }
     
%        \KwRet\;
  }

\caption{Constraints Inference - Associations}\label{algo:associations}
\end{algorithm}
   


==> data_synthesis.tex <==
\input{synthesis_algo}

\subsection{Realistic Data Synthesis}
\label{sec:Synth}
% This subsection discusses our overall approach to synthesize data in the structured form. The goal is to generate \textit{realistic} synthetic data which resembles the input data in terms of inherent distribution present in different features. To achieve this, we leverage the capabilities of our \emph{Constraint Inference} engine to uncover different distributions present in the data in the form of data constraints. We then synthesize data by making sure that the generated data satisfy these set of constraints to the best possible extent, as presented in Algorithm~\ref{algo:generate}. 
% The method \texttt{synthesize} in our algorithm expects two inputs: \textit{data} - a sample structured data, and \textit{n} - count of required number of synthetic tests to be generated.
% We then infer feature and association constraints for this input \textit{data} using \texttt{get\_constraints} method defined in Algorithm ~\ref{algo:generate}.
% Next, we describe the various components or functions used in Algorithm~\ref{algo:generate}.

This subsection discusses our overall approach to synthesize \textit{realistic} data using constraints inferred by \emph{Constraint Inference} engine (see Section~\ref{sec:spec}). The method \texttt{synthesize} in Algorithm ~\ref{algo:generate} expects two inputs: \textit{constraints} - data constraints for an input data, and \textit{n} - number of required synthetic tests to be generated.

Consider a toy dataset with three attributes (\texttt{gender(CAT\_TEXT), salary(FLOAT), age(NUMERIC)} with the following types of associations between them.
\begin{center}
\scriptsize
\begin{tabular}{cccc}
assoc-id & src & tgt & assoc-type \\
\hline
a1 & gender & age & CAT-NUM \\ 
a2 & age & salary & NUM-NUM \\
a3 & gender & salary & CAT-NUM \\
a4 & gender & education & CAT-CAT\\
a5 & education & gender & CAT-CAT\\
\hline
\caption{Associations}
\end{tabular}
\end{center}\\ 

In order to generate values for this example, we need to consider the following set of constraints.
\begin{enumerate}
    \item Feature Constraints of individual attributes
    \begin{itemize}[leftmargin=*]
        \item \emph{Continuous Distribution} in case of \texttt{NUMERIC} and \texttt{FLOAT}\\
        If values of \texttt{age} follows a normal distribution with specific bounds, we can sample required number of age values from this distribution using existing techniques.
        \item \emph{Discrete Distribution} followed by \texttt{CAT\_TEXT} and \texttt{CAT\_NUM}\\ Generation of values for \texttt{gender} in a fixed frequency ratio, say M:F=2:1, can done by using an existing solver.
        \item \emph{Regular Expression} captured by \texttt{TEXT}\\
        Generation of text values satisfying a pattern along with minimum and maximum length bounds can be achieved by existing methods.
    \end{itemize}
    \item Association Constraints
        \begin{itemize}[leftmargin=*]
            \item \emph{Polynomial Relationship} in case of \texttt{NUM-NUM} and \texttt{DATE-DATE}\\
            To generate values for \texttt{age} and \texttt{salary} such that they satisfy a polynomial equation, we can use any existing constraint solver.
            \item \emph{Joint Continuous Distribution} captured by \texttt{CAT-NUM} \\
            For \texttt{gender=M}, if salary follows a uniform distribution with specific bounds, then for every \texttt{M} value, we can sample a value from this distribution for \texttt{age}.
            \item \emph{Joint Discrete Distribution} in case of \texttt{CAT-CAT} \\
            For \texttt{gender=F}, if frequency distribution of \texttt{education} values, say masters:primary=20\%:80\%, then we first fetch the total count of \texttt{F} values in \texttt{gender}, say $10$. Therefore, $2$ females are assigned masters while $8$ are assigned primary as \texttt{education}.
        \end{itemize}
\end{enumerate}

But, the interesting part lies in how we try to generate values for an attribute while considering multiple constraints at once.
% Next, we describe the various components or functions used in Algorithm~\ref{algo:generate}.

\paragraph{Dependent Features.} Let us start with \texttt{is\_independent} method in Algorithm~\ref{algo:generate}. If a feature is specified as a target in any association in the fetched set of constraints, only then it's classified as dependent. As per our toy example, only \texttt{gender} is independent.

\paragraph{Feature Process Order.} We employ a column-wise generation scheme, where we generate data for independent features prior to the dependent ones. This ensures that at the time of generating column values for a dependent feature, the required source feature values have already been generated and are ready to be consumed. Therefore, \texttt{get\_process\_order} method analyzes the source and target features in all association constraints and results an order in which values for different features are to be generated. The process starts with creating a graph where all features are represented as nodes, and for every association constraint between source \textit{src} and target feature \textit{tgt}, a directed edge from node \textit{src} to \textit{tgt} is added in this graph. The graph then undergoes pre-processing to prune edges/associations in this graph.
\begin{figure}[t]
\centering
\includegraphics[width=8cm]{images/graph.png}
\caption{Associations Pruning}
\label{fig:graph}
\end{figure}
G1 in Figure~\ref{fig:graph} shows the association graph created for our exemplar dataset. Here, associations a4 and a5 form a cycle in the graph. But, in order to find the feature process order, we need an acyclic graph. Therefore, we \emph{break the existing cycles} or self loops in the graph by removing the last added edge/association in that cycle (i.e. a5). The resultant acyclic graph G2 is further looked for the cases where multiple transitive paths exist between two nodes, such as path (a1, a2) and (a3) between \texttt{gender} and \texttt{salary}. We \emph{remove such transitivity} by considering only the path with the shortest length and breaking the rest. Association a2 is therefore removed from graph G2 to yield final pruned set of association graph G3. The intuition behind considering shorter paths is to make sure that minimal approximation seeps from the source values to the target values while processing associations.
We then \emph{topologically sort} this directed acyclic graph G3 to return the order to process and generate values for the features, which in our case is \texttt{gender} followed by (\texttt{age, salary and education} in any order).


\paragraph{Generate by Feature Constraints.}  The method 
% \texttt{gen\_by\_feature\_constraints} 
at Line ~\ref{func:gen_by_features} in Algorithm ~\ref{algo:generate} concerns with generating values for an attribute by satisfying just the individual feature constraints based on their data types. No associations are considered here during the processing. As per the process order, \texttt{gender} is independent and hence its values will be generated by using feature constraints only. These values of \texttt{gender} will later act as source values while generating values for all its direct dependents using associations.
% Based on the datatype of the input feature, we generate values as follows.
% \begin{itemize}[leftmargin=*]
%     \item \textit{NUMERIC/FLOAT}: We generate the values for NUMERIC and FLOAT datatypes by drawing samples from the given statistical distribution in the feature constraint. Please note that apart from distribution name and parameters, we also consider minimum and maximum bounds along with the uniqueness constraints. In case where no distribution was inferred for the feature in the constraints, we use the default distribution as \emph{Uniform}.
%     \item \textit{CAT\_TEXT/CAT\_NUM}: For category related datatype, the constraints report the frequency distribution of different possible category values. We generate the values for a categorical feature such that they follow a similar relative frequency distribution as specified in the constraints. In case of unavailability of such constraint, we generate values by randomly picking values from the possible category value set.
%     \item \textit{TEXT}: Values for features with TEXT datatype are generated by satisfying the associated regex along with the minimum and maximum permissible lengths, and uniqueness constraints.
%     \item \textit{DATE}: We generate random date values between permissible start and end values for features with DATE datatype. Please note that while generating values, we do consider uniqueness constraints and output the values in the same date format as the one specified in the feature constraints.
% \end{itemize}

\paragraph{Generate by Associations.} For every dependent feature $f$, we begin with fetching all the association constraints with $f$ as target, refer line~\ref{line:assoc} in Algorithm~\ref{algo:generate}. The method at line~\ref{func:gen_by_assocs} concerns with processing and satisfying this subset of associations along with the feature constraints depending on the datatype of target feature $f$, as described next.
\begin{itemize}[leftmargin=*]
    \item \textit{NUMERIC/FLOAT}: As defined in \texttt{gen\_by\_numnum} at line~\ref{func:gen_by_numnum}, values can either be generated by constraint-solving or generative approach in case of NUM-NUM and CAT-NUM associations respectively. If NUM-NUM exists, then we first try to generate target values using NUM-NUM associations which are then validated against applicable distribution in CAT-NUM and NUM feature constraints. In case of existence of only CAT-NUM association, we sample a target value using one of the applicable distribution and validate if it fits the remaining CAT-NUMs and feature constraints. In case the validation of any generated value fails, we generate value using a fallback mechanism as per the following priority CAT-NUM $<$ NUM-NUM $<$ NUM feature constraints.
    \item \textit{CAT\_TEXT/CAT\_NUM}: As per \texttt{gen\_by\_catcat} at line~\ref{func:gen_by_catcat}, if an association of type CAT-CAT exists between two attributes, say education (source) and gender (target) such that for masters, male:female = 3:1, while for primary education, male:female = 1:1. Considering masters:primary = 1:1 in already generated 8 source values, we generate 3 (male, masters), 1 (female, masters), 2 (male, primary), 2 (female, primary) pairs in the synthetic tests. 
    \item \textit{DATE}: DATE\_DATE is the only type of association related to this datatype. The method \texttt{gen\_by\_datedate} at line~\ref{func:gen_by_datedate} in Algorithm~\ref{algo:synth_assocs} describes our way to satisfy such associations along with DATE related feature constraints simultaneously to generate data. Let's consider a toy dataset with two attributes OrderDate and DeliveryDate binded by the following constraints. \\
    \texttt{DeliveryDate = OrderDate + [2-10days]} (DATE-DATE)\\
    \texttt{15-05-1995 $\leq$ DeliveryDate $\leq$ Today} (Feature constraint) \\
    All these constraints for DeliveryDate are fed to a solver along with already generated values of OrderDate to yield DeliveryDate values which satisfy all these conditions.
\end{itemize}

\paragraph{Generate by considering User-Defined Constraints (UDCs)}
If user specifies some additional constraints to override the existing ones in data, then we first need to merge the two set of constraints, so that the resultant set comprises of non-conflicting constraints. This resultant merged constraint set is then used to synthesize test data by following the steps starting from line~\ref{line:process} in Algorithm~\ref{algo:generate}. 
% Merging of user-defined constraints (UDCs) with data constraints takes place in two consecutive steps - 
% \begin{enumerate}
%   \item \textit{Handle conflicts within the set of UDCs.} For any subset of conflicting constraints in user-defined set, we retain the one with the highest priority level in user-defined constraints and drop the rest.
%   \item \textit{Handle conflicts of filtered UDCs with the data constraints.} Please note that the UDCs have higher priority in case of any conflict with inferred data constraints. Following is our strategy to handle different types of UDCs.
UDCs are merged with data constraints by handling their conflicts  with the existing data constraints. Please note that the UDCs have higher priority in case of any conflict with inferred data constraints. Following is our strategy to handle different types of UDCs.
   \begin{itemize}[leftmargin=*]
    \item \textit{Add/Modify UDCs} - For every such UDC, we add/modify that constraint in our set of data constraints. In case of conflict, we record the over-riding constraints in our data constraints and make sure that the former get precedence over the latter during the synthesis process. \\
    - \emph{Range modification} - Please note that there is a need to handle the cases of range modification in a more systematic way. Consider a case where data constraints have a feature constraints on an attribute, say salary, where the values are bounded by range $(min_{data}, max_{data})$, say 2k-30k and follow a uniform distribution with certain parameters. Now, user specifies to override just the range for Salary as $(min_{user}, max_{user})$, say 5k-50k without any change in associated statistical distribution. Overriding just the bounds in the data constraints may impact the present distribution parameters. Therefore, using the original min-max bounds 2k-30k along with the specified uniform distribution parameters in the data constraints, we first generate a set of salary values, V. We then scale these generated values using the below formula for every value v $\in$ V to the final output values for salary. \\
    $
    v_{scaled} = min_{user} + \frac{(v - min_{data})*(max_{user}-min_{user})}{(max_{data}-min_{data})}
    $ \\
    This scaling ensures that the mean of scaled values is linearly scaled version of the values before scaling.
    \item \textit{Delete UDC} - We drop/disable such constraint from our set of data constraints. If the overriding constraints specify to drop an entire feature, $f$ from the resultant test set, then we drop the feature constraints along with all its related association constraints where $f$ is mentioned as either source or target.
\end{itemize}
% \end{enumerate}


==> disc.tex <==
\section{Industry Implications}
\label{sec:learning}



==> mymacros.tex <==
\usepackage{color}

\newtheorem{defn}{Definition}
\newcommand{\eat}[1]{} % comment
\newcommand{\remind}[1]{\textcolor{red}{\textsf{#1}}}


\newcommand{\BigCrunch}{\vspace{-1em}}
\newcommand{\Crunch}{\vspace{-0.8em}}
\newcommand{\SmallCrunch}{\vspace{-1ex}}
\newcommand{\Skip}{\vspace{1ex}}

\newcommand{\onefigure}[3]{
\begin{figure}[t]
\begin{center}
\centerline{\epsfxsize=0.98\columnwidth \epsffile{#1}}
\centerline{\parbox{\columnwidth}{\caption{#2} \label{#3}}}
\end{center}
\BigCrunch
\end{figure}
}

\newcommand{\onepdffigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.40]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}



\newcommand{\onelargepdffigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.37]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}

\newcommand{\onepdfigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.560]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}

\newcommand{\onesmallpdfigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.35]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}

\newcommand{\onemediumpdfigure}[3]{
    \begin{figure}[t] 
    \centerline{
    \includegraphics[scale=0.43]{#1}  
    }
    \vspace*{-1em}
    \centerline{
    \vspace*{-1.1em}
    \parbox{3.3in}{\caption{#2}
    \label{#3}}
    }
\end{figure}
}


\newcommand{\onetinyfigure}[3]{
\begin{figure}[t]
\begin{center}
\centerline{\epsfxsize=0.75\columnwidth \epsffile{#1}}
\centerline{\parbox{\columnwidth}{\vspace{-2em} \caption{#2} \label{#3}}}
\end{center}
\vspace{-4em}
\end{figure}
}

\newcommand{\onesmallfigure}[3]{
\begin{figure}[t]
\begin{center}
\centerline{\epsfxsize=0.85\columnwidth \epsffile{#1}}
\centerline{\parbox{\columnwidth}{\caption{#2} \label{#3}}}
\end{center}
\vspace{-2em}
\end{figure}
}


\newenvironment{my_enumerate}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}
{\end{enumerate}
}

\newenvironment{my_itemize}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}
{\end{itemize}
}

\newcommand{\twofigs}[6]{
\begin{figure*}[t]
\centerline{
            \epsfxsize=3.0in \epsffile{#1}
            \hfill
            \epsfxsize=3.0in \epsffile{#4}
           }
\centerline{
            \parbox{3.0in}{\caption{#2} \label{#3}}
            \hfill
            \parbox{3.0in}{\caption{#5} \label{#6}}
           }
\Crunch
\end{figure*}
}

\newcommand{\twolargefigs}[6]{
\begin{figure*}[t]
\centerline{
            \includegraphics[scale=0.4]{#1}
     \hfill
    \includegraphics[scale=0.7]{#4}
           }
\centerline{
            \parbox{3.5in}{\caption{#2} \label{#3}}
            \hfill
            \parbox{3.5in}{\caption{#5} \label{#6}}
           }
\end{figure*}
}
{\newcommand{\twofigures}[6]{
\begin{figure*}[tbh]
\centerline{
            %\hfill
            \includegraphics[scale=0.49]{#1}
            \hfill
            \includegraphics[scale=0.49]{#2}
            %\hfill
           }
\vspace*{-1ex}
            \parbox{3in}{\centering (a)}
    \parbox{3in}{\centering (b)}
%%\Crunch
\vspace*{-1ex}
\centerline{
            %\hfill
            \parbox{9.0in}{\caption{#3} \label{#4}}
            \hfill
          %%  \parbox{3.0in}{\caption{#5} \label{#6}}
          %%  %\hfill
           }
\Crunch
\end{figure*}
% \Skip
}


{\newcommand{\twolargefigures}[6]{
\begin{figure*}[tbh]
\centerline{
            %\hfill
            \includegraphics[scale=0.41]{#1}
            \hfill
            \includegraphics[scale=0.51]{#2}
            %\hfill
           }
\vspace*{-1ex}
            \parbox{3in}{\centering (a)}
    \parbox{3in}{\centering (b)}
%%\Crunch
\vspace*{-1ex}
\centerline{
            %\hfill
            \parbox{9.0in}{\caption{#3} \label{#4}}
            \hfill
          %%  \parbox{3.0in}{\caption{#5} \label{#6}}
          %%  %\hfill
           }
\Crunch
\end{figure*}
% \Skip
}


\newcommand{\twoabsinglecolumnfigures}[5]{
    \begin{figure}[!tbh]
    \centerline{
    \includegraphics[scale=0.2]{#1}
    \hfill
    \includegraphics[scale=0.2]{#2}
    }
    \parbox{0.45\columnwidth}{\centering (a) 10 node cluster}
    \parbox{0.45\columnwidth}{\centering (b) 30 node cluster}
    \centerline{
    \parbox{9in}{\caption{#3}
    \label{#4}}
    \hfill
    }
\vspace{-0.2in}
%\Crunch
%    \DoubleSpace
%\Skip
\end{figure}
}



\newcommand{\threefiguressmaller}[5]{
    \begin{figure*}[tbh]
    \centerline{
    \includegraphics[scale=0.37]{#1}
    \hfill
    \includegraphics[scale=0.37]{#2}
    \hfill
    \includegraphics[scale=0.37]{#3}
    }
\vspace{-0.6em}
%    \SingleSpace
     \parbox{2.31in}{\centering (a)}
    \parbox{2.46in}{\centering (b)}
    \parbox{2.4in}{\centering (c)}    \centerline{
    \parbox{9in}{\caption{#4}
    \label{#5}}
    \hfill
    %%\parbox{2.15in}{\caption{#5}
   %% \label{#6}}
   %% \hfill
    %%\parbox{2.15in}{\caption{#8}
   %% \label{#9}}
    }
\vspace{-0.2in}
%\Crunch
%    \DoubleSpace
%\Skip
\end{figure*}
}




\eat{\newcommand{\threefigures}[9]{
    \begin{figure*}[tbh]
    \centerline{
    \epsfxsize=2.4in \epsffile{#1}
    \hfill
    \epsfxsize=2.4in \epsffile{#4}
    \hfill
    \epsfxsize=2.4in
    \epsffile{#7}
    }
\vspace{-1em}
%    \SingleSpace
    \centerline{
    \parbox{2.15in}{\caption{#2}
    \label{#3}}
    \hfill
    \parbox{2.15in}{\caption{#5}
    \label{#6}}
    \hfill
    \parbox{2.15in}{\caption{#8}
    \label{#9}}
    }
\Crunch
%    \DoubleSpace
\Skip
\end{figure*}
}}

\newcommand{\fourfigures}[8]{
    \begin{figure*}[thb]
    \centerline{
    \epsfxsize=1.575in \epsffile{#1}
    \hfill
    \epsfxsize=1.575in \epsffile{#2}
    \hfill
    \epsfxsize=1.575in \epsffile{#5}
    \hfill
    \epsfxsize=1.575in \epsffile{#6}
    }
%    \SingleSpace
\SmallCrunch
    \centerline{
    \parbox{3.2in}{\caption{#3} \label{#4}}
    \hfill
    \parbox{3.2in}{\caption{#7} \label{#8}}
    }

%    \DoubleSpace
\Skip
\end{figure*}
}

\newenvironment{my_description}{
\begin{description}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}}
{\end{description}}

\newenvironment{mylist}{
% \baselineskip 10 pt
\begin{list}{$\bullet$}{
\setlength{\leftmargin}{1.5ex}
\setlength{\labelwidth}{1ex}
\setlength{\labelsep}{0.5ex}
\setlength{\itemsep}{0.2ex}
\setlength{\parsep}{0.2ex}
}}
{\end{list}}


==> palgo.tex <==
\begin{algorithm}
% \scriptsize
\footnotesize
% \small
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

\SetKwProg{Fn}{Function}{}{end}
\Fn{DataSynthesis(InputData, n)}{
    DataConstraints = genConstrains(InputData)\\
    CDG =  createCDG(DataConstraints)\\
    return DataSynWithDataCons(CDG, n)\\
}

\Fn{createCDG(DC, n)}{
    G.nodes = \{\}\\
    G.edges = \{\}\\
    \ForEach{$c \in DC.columns$}{
        G.nodes += $n_c$
    }    
    \ForEach{$fc \in DC.feature\_constraints$}{
        $n_c.constraints$ += $fc$\\ 
        \uIf{($n_c.type == NUM \wedge \exists c \in fc~s.t.~c.type==cont\_distribution$)}{
            $n_c.GenNode = False$
        }\Else{
            $n_c.GenNode = True$
        }
    }    
    \ForEach{$ac \in DC.assoc\_constraints$}{
        $n_c.asso\_constraints$ += $ac$ 
    }
    return G
}
\Fn{DataSynWithDataCons(CDG, n)}{
    DAG = preProcess(CDG)\\
	return generate(DAG, n)			
}
\Fn{preProcess(CDG)}{
    DAG = CDG.copy()\\
    \While{$\exists~directed~cycle~$c$ \in DAG$}{
        delete edge ($n_i,n_j$) with minimal confidence s.t. $n_j.GenNode = True$
    }
    return DAG
}

\Fn{DataSynWithDataCons(DAG, n)}{
    \While{$n_j \in topologicalOrder(DAG.nodes)$}{
        data = genDataEachColumn($n_j$, DAG, n)\\
        $n_j.data = data$
    }
}
\Fn{genDataEachColumn($n_j$, DAG, n)}{
        \uIf{($n_j.GenNode \wedge n_j.type == NUM$)}{
            dataOwn = gen($n_j$.dist, n, $n_j$.range, $n_j$.isUnique)\\
            minDiv = +Inf\\
            minDivData = null\\
            \ForEach{(e = ($n_i$,$n_j$)}{
                data=genData(e,$n_i$)\\          
                div = KL-div(dataOwn, data) \\    
                \If{$div < minDiv$}{
                    minDivData = data\\
                }
            }
            $n_j.data = data$\\
        }\uElseIf{($n_j.GenNode$)}{ \tcp*[l]{type CAT}
            e = ($n_i$,$n_j$) for any $n_i$\\
            data=genData(e,$n_i$)\\          
            $n_j.data = data$\\
        }\Else{\tcp*[l]{NonGenNode}
            e = ($n_i$,$n_j$) s.t. $error(e)$ is min for all $n_i$\\
            data=genData(e,$n_i$)\\          
            $n_j.data = data$\\
        }
    }
}

\caption{Data Synthesis using Data Constraints}
\label{algo:ds}
\end{algorithm}

==> property_tds.tex <==

\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

    \SetKwFunction{FMain}{synthesize}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{train\_data, n, class\_label, property, protected\_attr=None}}{ \label{func:synthesize}
        constraints = get\_constraints(train\_data) \\
        feature\_order = get\_process\_order(constraints, class\_label, property, protected\_attr)\\
       //same as lines ~\ref{line:st}-~\ref{line:ed} in Algorithm ~\ref{algo:generate} \\
        \KwRet synth\_data
    }
  
    \SetKwFunction{FMain}{get\_process\_order}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{constraints, class\_label, property, protected\_attr=None}}{ \label{func:gpo_prop}
        constraints.remove\_feature(class\_label)\\ \label{line:label}
        \uIf{property $\in$ \{GROUP\_FAIRNESS\}}{ \label{line:fair}
            constraints.remove\_associations(protected\_attr)
        }
        g = create\_graph(constraints.feature\_names)\\
        g.add\_all\_edges(constraints.associations)\\
        g = preprocess(g)\\
        feature\_order = topological\_sort(g)\\
        \KwRet feature\_order
    }

\caption{Property based Test Input Generation}\label{algo:fairness}
  
\end{algorithm}

As mentioned in Section~\ref{sec:arch}, we further intend to generate realistic test cases to test an input AI model for a number of properties, namely, \emph{Correctness}, \emph{Individual Fairness}, \emph{Group Fairness} and \emph{Robustness}. We use the same base approach as presented above with a few changes depending on the property. The required algorithmic changes are concerned only with the user inputs, and the implementation of method \texttt{gen\_process\_order}, as presented in Algorithm ~\ref{algo:fairness}. Following are the user inputs required for property-based test inputs generation to test an AI model.
\begin{itemize}
    \item \textit{data} - training data from which data constraints are fetched.
    \item \textit{n} - count of required test inputs to be generated.
    \item \textit{class\_label} - feature name in the input data containing the decision class values.
    \item \textit{property} - AI model test property for which test inputs need to be generated.
    \item \textit{protected\_attr} - name of the protected or sensitive attributes such as gender, race, etc. present in the input training data, based on which the input AI model is not supposed to take any decision in an ideal scenario. Please note that this is a mandatory user input only for Individual and Group Fairness property use cases. 
\end{itemize}
For the property based test input generation given in Algorithm ~\ref{algo:fairness}, the method \texttt{gen\_process\_order} starts with removing the feature related to input class label along with all the association constraints where this feature is specified as either a source or target (line ~\ref{line:label}). This is done to make sure that any approximation caused due to constraint inference or synthesis does not seep into the prediction labels for these test inputs.

\subsubsection{Correctness Test Case Generator}
Since we generate test inputs conforming to the behaviour/constraints inherent in the input training data, therefore, these realistic test inputs, of reasonably good size, should be able to cover most of the paths of the trained model. Hence, they can be put to test correctness of an input AI model too. As mentioned earlier, we don't use constraints to synthesize prediction values for these realistic test cases. Label assignment ideally should be a done by manual intervention, but, we instead use a \emph{Multi-model Label Generator} to guess labels for these inputs.
\input{label_generator}


\subsubsection{Individual Fairness Test Case Generator}
As mentioned earlier in Section~\ref{sec:back}, we employ an existing approach \cite{testing-fse} to generate test cases for individual fairness testing of a black-box AI model. The process of generation involves the following two phases.\\
\textit{Global Search} - First, we synthesize required number of test cases by satisfying data constraints, which constitute the set of global inputs. \\ 
\textit{Local Search} - The global inputs are then clustered and processed one by one according to the strategy in \cite{testing-fse}. Once a discriminatory test case, say t, is found, we try to generate further more test inputs in its neighborhood which may lead to uncover individual discrimination. 
We use an off-the-shelf explainer LIME~\cite{LIME} to get a set of top $50\%$ attributes contributing to the explanation of test case, t. For every prominent attribute, say a, we then generate further more local test inputs by perturbing its value as per the below scheme based on its datatype.\\
\emph{CAT\_TEXT/CAT\_NUM}: Generate inputs by perturbing t[a] for all possible values. \\
\emph{NUMERIC/FLOAT}: Generate inputs by perturbing t[a] for all integers or floats in range (t[a]-3, t[a]+3). Please note that the perturbation in such cases are bounded by the minimum and maximum permissible bounds of attribute a inferred from data constraints.
\subsubsection{Group Fairness Test Case Generator} 
Specifically just for the group fairness use case, in addition to class label, we further unconditionally make the protected feature independent by removing all those associations from the data constraints where it is mentioned as the target (line ~\ref{line:fair}). This is done to ensure that the protected attribute in resultant synthetic test inputs follow the same frequency distribution as that of the input training data set. For example, if the training data has composition of males and females in the ratio 2:1, then, it is desirable to test the model for group fairness with the test cases having same 2:1 male female ratio. Please note that this frequency distribution of protected attribute can be over-ridden by means of user-specified constraints as well as mentioned earlier in Subsection~\ref{sec:user-defined}.
\subsubsection{Robustness Test Case Generator}
Except for the class label, we synthesize realistic data satisfying all the feature and association constraints. For every realistic test, say t, we then perform robustness testing of the input model by generating more inputs in its neighbourhood, and checking if the predictions of any neighbour is different than t's. Please note that we use the same definition of neighborhood as the one used in Individual Fairness Test Generator.

==> synthesis_algo.tex <==
\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

\SetKwFunction{FMain}{synthesize}
  \SetKwProg{Fn}{function}{:}{}
  \Fn{\FMain{constraints, n}}{ \label{func:synthesize}
        % constraints = get\_constraints(data) \\
        feature\_order = get\_process\_order(constraints)\\ \label{line:process}
        synth\_data = \{ \}\\ \label{line:st}
        \ForEach {feature $f$ in feature\_order}{
            \uIf{is\_independent(f, constraints)}{
                synth\_vals = gen\_by\_feature\_constraints(f, n)
            }
            \uElse{
            assocs = constraints.get\_all\_associations(f) \\ \label{line:assoc}
 synth\_vals = gen\_by\_associations(f, assocs, synth\_data, n)
            }
            synth\_data[f] = synth\_vals 
        } \label{line:ed}
        \KwRet synth\_data
    }
  
    \SetKwFunction{FMain}{get\_process\_order}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{constraints}}{ \label{func:get_order}
        g = create\_graph(constraints.feature\_names)\\
        g.add\_all\_edges(constraints.associations)\\
        g = preprocess(g)\\
        feature\_order = topological\_sort(g)\\
        \KwRet feature\_order
    }
    
    \SetKwFunction{FMain}{is\_independent}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{feature, constraints}}{ \label{func:get_order}
        assocs = constraints.get\_all\_associations(feature)\\
        \uIf{ assocs is None}{
            \KwRet True
        }
        \KwRet False
    }


    \SetKwFunction{FMain}{gen\_by\_feature\_constraints}
    \SetKwProg{Fn}{function}{:}{}
    \Fn{\FMain{feature $f$, n}}{ \label{func:gen_by_features}
        \uIf{f.datatype $\in$ \{NUMERIC, FLOAT\}}{
            dist = f.distribution\\
            \uIf{dist is None}{
                vals = draw\_samples(UNIFORM, f.min, f.max, f.is\_unique, n)
            }
            \uElse{
            vals = draw\_samples(dist.name, dist.parameters, f.min, f.max, f.is\_unique, n)
            }
        }
        \uElseIf{feature.datatype $\in$ \{CAT\_TEXT or CAT\_NUM\}}{
            \uIf{feature.frequency is None}{
            vals = gen\_randomly(f.possible\_vals, n)
            }
            \uElse{
            vals = gen\_by\_freqDist(f.frequency, n)
            }
        }
        \uElseIf{feature.datatype is TEXT}{
            vals = gen\_by\_regex(f.pattern, f.min\_len, f.max\_len, f.is\_unique, n)
        }
        \uElseIf{feature.datatype is DATE}{
            vals = gen\_dates\_between(f.start\_date, f.end\_date, f.format, 
            f.is\_unique, n)
        }
        \KwRet vals
    }

\SetKwFunction{FMain}{gen\_by\_associations}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, assocs, synth\_data, n}}{ \label{func:gen_by_assocs}
    \uIf{feature.datatype $\in$ \{NUMERIC, FLOAT\}}{
        numnum\_assocs = assocs.get\_by\_type(NUM-NUM)\\
        catnum\_assocs = assocs.get\_by\_type(CAT-NUM)\\
        \uIf{numnum\_assocs is not None}{
            vals = gen\_by\_numnum(f, numnum\_assocs, assocs, synth\_data, n)\\
         }
        
        \uElseIf{catnum\_assocs is not None}{
            vals = gen\_by\_catnnum(f, catnum\_assocs, synth\_data, n)\\
        }
        
    }
    \uIf{feature.datatype $\in$ \{CAT\_TEXT, CAT\_NUM\}}{
        vals = gen\_by\_catcat(f, assocs, synth\_data, n)\\
    }
    
    \uIf{feature.datatype is DATE}{
        vals = gen\_by\_datedate(f, assocs, synth\_data, n)\\
    }
    \KwRet vals
}

\caption{Realistic Data Synthesis}\label{algo:generate}
  
\end{algorithm}




\begin{algorithm}[htb]
\scriptsize
\SetAlgoLined
\SetAlgoLined\DontPrintSemicolon

\SetKwFunction{FMain}{gen\_by\_numnum}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, numnum\_assocs, catnum\_assocs, synth\_data, n}}{ \label{func:gen_by_numnum}
    solver = Solver()\\
    \ForEach{assoc $\in$ numnum\_assocs}{
             equations = form\_equations(assoc, synth\_data[assoc.source])\\
             solver.add(equations)\\
    }
     vals = solver.solve(f.is\_unique)\\
     
     isValid, invalid\_idxs = validate(val, catnum\_assocs, feature)\\
        \uIf{!isValid}{
            \ForEach{idx $\in$ invalid\_idxs}{
                vals[idx] = gen\_by\_catnum($f$, catnum\_assocs, synth\_data, n=1)
            }
        }
     \KwRet vals
}

\SetKwFunction{FMain}{gen\_by\_catnum}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, catnum\_assocs, synth\_data, n}}{ \label{func:gen_by_catnum}
        vals = []\\
        \ForEach{srcval $\in$ synth\_data[assoc.source]}{
            assoc = pick\_max\_overlap\_catnum(catnum\_assocs, srcval) \\
            dist = assoc.get\_dist\_by\_src(srcval)\\ trials=0, success=False\\
            \While{!success and trials < MAX\_TRIALS}{
                val = draw\_samples(dist.name, dist.parameters,f.min,f.max, n=1)\\
                \uIf{f.is\_unique and is\_exists(val, vals)}{
                    trails++, continue
                }
                isValid = validate(val, catnum\_assocs, feature)\\
                \uIf{isValid}{success=True}
                trail++
            }
            \uIf{!success}{
                val = gen\_by\_feature\_constraints(feature=f, n=1)
            }
            vals.append(val)
        }
}


\SetKwFunction{FMain}{gen\_by\_catcat}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, assocs, synth\_data, n}}{ \label{func:gen_by_catcat}
    assoc = pick\_any\_randomly(assocs) \\
    src\_vals = synth\_data[assoc.source]\\
    vals = gen\_by\_freq(assoc.frequency, src\_vals) \\
    \KwRet vals
}



\SetKwFunction{FMain}{gen\_by\_datedate}
\SetKwProg{Fn}{function}{:}{}
\Fn{\FMain{feature $f$, assocs, synth\_data, n}}{ \label{func:gen_by_datedate}
    \ForEach{assoc $\in$ assocs}{
        src\_vals = synth\_data[assoc.source]\\
        solver = datesolver(), i=0\\
        \While{i $<$ n}{
            solver.add($val_{i}$ $==$ $src\_val_{i}$ $+$ $delta_{i}$)\\
            solver.add($delta_{i}$ $>=$ $assoc.min\_diff$)\\
            solver.add($delta_{i}$ $<=$ $assoc.max\_diff$)\\
            solver.add($val_{i}$ $>=$ $f.start\_date$)\\
            solver.add($val_{i}$ $<=$ $f.end\_date$), i++\\
         }
        } 
    
    vals = solver.solve(unique=f.is\_unique), i=0 \\
    //fallback\\
    \While{i $<$ n}{     
        \uIf{$vals[i]$ is None}{
            vals[i] = gen\_by\_feature\_constraints(f, n=1)
        }
    }
    \KwRet vals
    }
}


\caption{Synthesis Using Associations} \label{algo:synth_assocs}
\end{algorithm}
